Workflows Community Summit: Bringing the Scientific Workflows Community Together

Scientific workflows have been used almost universally across scientific domains, and have underpinned some of the most significant discoveries of the past several decades. Many of these workflows have high computational, storage, and/or communication demands, and thus must execute on a wide range of large-scale platforms, from large clouds to upcoming exascale high-performance computing (HPC) platforms. These executions must be managed using some software infrastructure. Due to the popularity of workflows, workflow management systems (WMSs) have been developed to provide abstractions for creating and executing workflows conveniently, efficiently, and portably. While these efforts are all worthwhile, there are now hundreds of independent WMSs, many of which are moribund. As a result, the WMS landscape is segmented and presents significant barriers to entry due to the hundreds of seemingly comparable, yet incompatible, systems that exist. As a result, many teams, small and large, still elect to build their own custom workflow solution rather than adopt, or build upon, existing WMSs. This current state of the WMS landscape negatively impacts workflow users, developers, and researchers. The "Workflows Community Summit" was held online on January 13, 2021. The overarching goal of the summit was to develop a view of the state of the art and identify crucial research challenges in the workflow community. Prior to the summit, a survey sent to stakeholders in the workflow community (including both developers of WMSs and users of workflows) helped to identify key challenges in this community that were translated into 6 broad themes for the summit, each of them being the object of a focused discussion led by a volunteer member of the community. This report documents and organizes the wealth of information provided by the participants before, during, and after the summit.

==> _format.tex <==
%%%%% Title Spacing and Format %%%%%%
\titlespacing{\section}{0pc}{1pc}{1pc}
\titlespacing{\subsection}{0pc}{2pc}{1pc}
\titlespacing{\subsubsection}{0pc}{1pc}{1pc}
\titleformat*{\section}{\Large\bfseries}
\titleformat*{\subsection}{\large\bfseries}
\titleformat*{\subsubsection}{\normalsize\bfseries}

%%%%% Margins %%%%%%%%%%%%%%%%%%%%%%%%
\pagestyle{plain}
\setlength{\textwidth}{6.5in}
\setlength{\oddsidemargin}{0in}
\setlength{\evensidemargin}{0in}
\setlength{\textheight}{8.3in}
\setlength{\topmargin}{0in}
\setlength{\headheight}{0in}
\setlength{\headsep}{.3in}
\setlength{\footskip}{.5in}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \SetWatermarkText{\textsc{Draft}}
% \SetWatermarkScale{0.75}
% \SetWatermarkColor[gray]{0.9}

\lstdefinestyle{wcsStyle}{
  tabsize=4,
  showspaces=false,
  showstringspaces=false,
  aboveskip=0em,
  belowskip=0em,
}


==> _headers.tex <==
\pagestyle{fancy}
\fancyhf{}
\rhead{
  \includegraphics[height=12pt]{figures/workflowsri-horizontal.png} %\ \ \
  \includegraphics[height=11pt]{figures/exaworks-horizontal.png}
}
\lhead{2021 Workflows Community Summit}
\rfoot{\thepage}


==> _macros.tex <==

\newcommand{\TODO}[2][inline]{\todo[color=red!50,#1]{\textbf{TODO:} #2}\xspace}
\newcommand{\rafael}[2][inline]{\todo[color=green!50,#1]{\textbf{Rafael F. Da Silva:} #2}\xspace}
\newcommand{\HC}[2][inline]{\todo[color=green!50,#1]{\textbf{Henri Casanova:} #2}\xspace}
\newcommand{\kyle}[2][inline]{\todo[color=green!50,#1]{\textbf{Kyle Chard:} #2}\xspace}
\definecolor{Gray}{gray}{0.9}

\renewcommand{\contentsname}{\\\hfill \large Table of Contents \hfill}
\newcommand{\pp}[1]{\medskip \noindent \textbf{\emph{#1.}}\xspace}


==> _packages.tex <==
\usepackage{times}
\usepackage{relsize}
\usepackage{microtype}
\usepackage{cite}
\usepackage{xspace}
\usepackage[table,xcdraw]{xcolor}
\usepackage{color,colortbl}
\usepackage{subfigure}
\usepackage{alltt}
\usepackage{url}
\usepackage{comment}
\usepackage{graphicx}
\usepackage{relsize}
\usepackage{paralist}
\usepackage{todonotes}
\usepackage{wrapfig}
\usepackage{titlesec}
\usepackage{epsfig}
\usepackage{geometry}
\usepackage{tikz}
\usepackage[normalem]{ulem}
\usepackage{titlesec}
\usepackage{booktabs}
\usepackage{wrapfig}
\usepackage{multirow}
\usepackage{pifont}
\usepackage{wrapfig}
\usepackage{soul}
\usepackage{enumitem}
\usepackage{tcolorbox}
\usepackage{pdfpages}
% \usepackage{hyperref}
\usepackage{fancyhdr}
\usepackage{longtable}
\usepackage{makecell}
\usepackage{lettrine}
% \usepackage{draftwatermark}
\usepackage{listings}


==> _references.tex <==
\newpage
\cleardoublepage\phantomsection\addcontentsline{toc}{section}{References}
\bibliographystyle{IEEEtran}
\bibliography{references}

